The Number of Large Graphs with a Positive Density of Triangles

We give upper and lower bounds on the number of graphs of fixed degree which have a positive density of triangles. In particular, we show that there are very few such graphs, when compared to the number of graphs without this restriction. We also show that in this case the triangles seem to cluster even at low density.

==> triang.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point       1.25       2.15 {\llap{$a$}}
\point       4.35       2.85 {\llap{$b$}}
\point       3.05       0.55 {\llap{$c$}}
\point       8.75       2.15 {\llap{$a$}}
\point      11.85       2.85 {\llap{$b$}}
\point      10.55       0.55 {\llap{$c$}}
\point       2.95      -0.45 {\clap{$R$}}
\point      10.45      -0.45 {\clap{$F$}}
 }}


==> xdefs3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% mechanism for forward referencing %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\catcode`\@=11
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% This checks whether the defs.lst file contains
%% at least the line
%% \def\nonemeptydefs{}
%% which was written by xdefs
%% Otherwise, we assume 
%% that defs.lst must be completely recreated.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@checkfirstline{\ifundefined{nonemptydefs}
\gdef\@haddefs{F}
\immediate\write16{--------Recreating defs.lst}
\else
\gdef\@haddefs{T}
\immediate\write16{--------Using old defs.lst}
\fi
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% define a new symbol%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@definereally#1#2#3{\expandafter\xdef\csname #1#2\endcsname{#3}\relax}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  write defined symbol to file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@writetofile#1#2#3{%
\write\@defs{\string\expandafter\string\xdef\string\csname}\relax%%
\write\@defs{\string #1#2\string\endcsname{\csname #1#2\endcsname}}}%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% check whether defs.lst exists%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\gdef\@haddefs{T}
\gdef\@neednewrun{T}
\gdef\@erasedefs{F}
\gdef\@doubly{F}
\newread\@defs
\openin\@defs defs.lst
\ifeof\@defs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% it does not exist%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\gdef\@haddefs{F}
\immediate\write16{*********Creating defs.lst}
\else
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% it exists and now we check if its ``empty''%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\closein\@defs
\input defs.lst
\@checkfirstline
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% now we open it for writing again%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\openout\@defs=defs.lst%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% ... and we write the identification line%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\write\@defs{\string\def\string\nonemptydefs{}}%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% @phaseone creates definitions when defs.lst is recreated from scratch%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@phaseone(#1,#2,#3){\ifundefined{#1#2}%%
\@definereally{#1}{#2}{#3}%%
\@writetofile{#1}{#2}{#3}%%%
\else%%
 \write16{!!!!!doubly defined #1,#2}%%
 \gdef\@doubly{T}%%
\fi%%
}%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% @phasetwo creates definitions when defs.lst existed.%%
%% it also checks if the definition of the value of a symbol%%
%% has changed (e.g. if the euqtion was moved inside the paper)%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@phasetwo(#1,#2,#3){\@undefineda{#1#2}%%
\else%%
\edef\@firstarg{\csname #1#2\endcsname}%%
\edef\@secondarg{#3}%%
\ifnum \@stringcompare{\@firstarg}{\@secondarg} = 0%%
\else%%
\immediate\write16{ definition of #1 #2 changed : \@firstarg  --->\@secondarg}%%
\gdef\@neednewrun{T}%%
\gdef\@erasedefs{T}%%
\fi%%
\fi%%
\@definereally{#1}{#2}{#3}%%
\@writetofile{#1}{#2}{#3}}%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% check if symbol was never defined (used when defs.lst already exists)%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@undefineda#1{\expandafter\ifx\csname#1\endcsname\relax%%%
{\gdef\@neednewrun{T}%%
 \immediate\write16{*********** used #1 which was never defined }}}%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% redefinition of NEWDEF depending on whether defs existed%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\if F\@haddefs%%
 \def\NEWDEF#1#2#3{\@phaseone({#1},{#2},{#3})}%%
\else%%
 \def\@neednewrun{F}%%
 \let\ifundefined=\@undefineda%%
 \def\NEWDEF#1#2#3{\@phasetwo({#1},{#2},{#3})}%%
\fi%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% messages when \bye is encountered (you cannot use \end)%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\bye{\if T\@erasedefs%%
 \write16{**** I suspect doubly defined tokens ****}%%
 \write16{**** I erase defs.lst now ***********}%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% next line ``erases'' defs.lst so that it will be%%
%% recreated in the next run%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \openout\@defs=defs.lst%%
\fi%%
\if T\@doubly%%
 \write16{**** There are doubly defined tokens *****}%%
 \write16{**** You have to correct the TeX file and rerun *****}%%
\fi%%
\if T\@neednewrun%%
 \write16{*********NEED ANOTHER RUN************}%%
\fi%%
\end}%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@stringcompare#1#2{\expandafter\@strcompa#1|===#2|===}%%
\def\@strcompa#1===#2==={\expandafter\@strcompb#2===#1===}%%
\def\@strcompb#1===#2==={\@compcont#1\\#2\\}%%
\def\@compcont#1#2\\#3#4\\{%%%
\csname @comp%%%
 \if #1#3\if #1|same\else contt\fi%%
   \else diff\fi%%
  \endcsname #2\\#4\\}%%
\def\@compcontt#1#2\\#3#4\\{\@strcompb#1#2===#3#4===}%%
\def\@compsame#1\\#2\\{0}%%
\def\@compdiff#1\\#2\\{1}%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\catcode`\@=\active
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% EOF xdefs.tex %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
